Breaking-Good: Explaining Breaking Dependency Updates with Build Analysis

Dependency updates often cause compilation errors when new dependency versions introduce changes that are incompatible with existing client code. Fixing breaking dependency updates is notoriously hard, as their root cause can be hidden deep in the dependency tree. We present Breaking-Good, a tool that automatically generates explanations for breaking updates. Breaking-Good provides a detailed categorization of compilation errors, identifying several factors related to changes in direct and indirect dependencies, incompatibilities between Java versions, and client-specific configuration. With a blended analysis of log and dependency trees, Breaking-Good generates detailed explanations for each breaking update. These explanations help developers understand the causes of the breaking update, and suggest possible actions to fix the breakage. We evaluate Breaking-Good on 243 real-world breaking dependency updates. Our results indicate that Breaking-Good accurately identifies root causes and generates automatic explanations for 70% of these breaking updates. Our user study demonstrates that the generated explanations help developers. Breaking-Good is the first technique that automatically identifies causes of a breaking dependency update and explains the breakage accordingly.

==> old-text.tex <==

% \begin{listing}

% \begin{minted}[fontsize=\scriptsize, frame=single,
%                framesep=2.0mm]{text}
% [INFO] ----------------------------------------------
% [WARNING] COMPILATION WARNING : 
% [INFO] ----------------------------------------------
% [WARNING] bootstrap class path not set in conjunction
% with -source 8
% [INFO] 1 warning
% [INFO] ----------------------------------------------
% [INFO] ----------------------------------------------
% [ERROR] COMPILATION ERROR : 
% [INFO] ----------------------------------------------
% [ERROR] /flink-faker/src/main/java/com/github/
% knaufk/flink/faker/DateTime.java:[43,3] method
% does not override or implement
% a method from a supertype
% [ERROR] /flink-faker/src/main/java/com/github/
% knaufk/flink/faker/DateTime.java:[45,40] 
% incompatible types: java.util.Date cannot 
% be converted to java.sql.Timestamp
% [INFO] 2 errors 
% [INFO] ----------------------------------------------
% [INFO] ----------------------------------------------
% [INFO] BUILD FAILURE
% [INFO] ----------------------------------------------
% [INFO] Total time:  35.243 s
% [INFO] Finished at: 2023-07-23T00:53:28Z
% [INFO] ----------------------------------------------
% \end{minted}
% \caption{An example log file snippet for \emph{Compilation failure}} 
% \label{lst:example-log-compilation-failure}
% \end{listing}


Fault localization is essential for identifying and isolating the root causes of problems in projects created with Maven, enabling efficient debugging and resolution \cite{Luis2012ASpecifications,flacoco2021,ReidemeisterFault,Khan2023ImpactDetection,Shin2021ADetection}.


\subsection{XXXX}

%Explaining 
Recent research approaches the generation of explanations for build failures.
As highlighted in the study by Kochhar et al. \cite{Kochhar2016PractitionersLocalization}, fault localization must provide justification; however, studies offering a direct explanation of the faulty line are still limited.
Groce \cite{groce2005error} discusses the challenge of debugging in software development, highlighting the difficulty of understanding and correcting compilation errors. The study introduces an approach called error explanation, which utilizes distance metrics for program executions to provide automated assistance.
Qiuping \etal \cite{Yi2015ExplainingLocalization} proposes CaFL, a cascade fault localization method, which systematically computes potential causes of software failures, augments them with contextual information, and organizes them into a tree structure for efficient pruning, significantly expediting the debugging process.

Breaking good generates explanations of build failures based on information retrieved from Maven build logs, including the causes of the failure and the affected client-side instructions.


\subsection{Compilation failures}
\label{sec: compilation_failures}
% Compilation failures are situations in which the source code cannot be correctly converted into executable code due to syntactic or semantic problems.
We consider a breaking dependency update as a \emph{Compilation failure} if the reproduction fails due to compilation failures. We identify a compilation failure from a log file if it contains the clause \emph{"COMPILATION ERROR:"}.
For example, if the log file contains the snippet given in \autoref{lst:example-log-compilation-failure}, we consider it a compilation failure. This indicates that the dependency update has introduced syntactical errors in the project code.

In the following section, we will explore four specific types of explanations for different types of compilation failures: Werror, Compilation failures, External dependencies, and Java incompatibilities. Each explanation provides important information for identifying and fixing compilation failures effectively. 

\subsubsection{Kind of suggestions} 
\label{suggestions}



    \textbf{Werror:} During compilation, the compiler generates warnings to alert about potential problems or non-standard usage that could cause errors or unexpected behavior at runtime. 
    
    \textbf{Compilation failures}
    
     \textbf{External dependencies}
     
    \textbf{ Java incompatibility}


We rely on the third-party tool \href{https://github.com/siom79/japicmp}{japicmp} to identify these changes.
\emph{japicmp} uses static analysis to identify changes between two versions of jar \todo{elaborate a bit on the type of analysis. does it analyze bytecode or src code? what kind of diff algo does it use?}.
This tool detects changes such as \todo{a word is missing here} (e.g., fieldRemoved, methodRemoved), changes in modifiers (e.g., methodNowAbstract, classNowFinal) and visibility (e.g., fieldLessAccessible), and changes in type (e.g., methodReturnTypeChanged).





% \emph{the root cause of the breakage is in one indirect dependency that affects the behavior of the direct dependency that has been updated}
% \emph{Analyze differences in the transitive dependencies}

% We retrieve the complete list of transitive dependencies for the new and previous versions of the updated dependency and compare both lists.
% From this comparison, each transitive dependency is in one of the following situations: no changes, deleted, added, or updated.

% If a dependency has been added or removed from the list of transitive dependencies, then we analyze whether the breakage is due to the use of deleted dependency constructs or incompatible constructs defined in the new transitive dependencies. 
% For instance, the project \texttt{docker-adapter} build fails to update the \texttt{http} dependency from version \texttt{v0.25} to version \texttt{v1.1.0} because the \texttt{org.cactoos} dependency was removed from version \texttt{v1.1.0}.

% When some transitive dependencies have been updated in the new version, we analyze which constructs change in the new version of each updated transitive dependency.
% As a result, we obtain a complete list of all modified constructs.
% Subsequently, we examine whether the components causing the breakage update belong to any of the transitive dependencies that have been updated.
% For example, the update of  \texttt{logback-classic} from version \texttt{1.2.11} to version \texttt{1.4.1} in the \texttt{pay-adminusers} project fails the build because it is not possible to load the \texttt{org.slf4j.spi.LoggingEventAware} class from the transitive dependency \texttt{slf4j-spi}.
    

\subsection{Analyze the two dependency versions}

We aim to analyze changes between versions of dependencies that lead to breaking updates.
We inspect modifications to methods, classes, and other constructs to detect potential compatibility issues.

We automatically analyze the bytecode of the new version of the dependency to find out which elements have been removed or modified compared to the previous version.
As a result, we obtain a list of all the constructs that have been modified in the new version. 
In most cases, a subset of these modified constructs can be found in the client and serves as a basis to generate an explanation.
Referring to the example in \autoref{fig:bdu_example}, when comparing both versions of the \texttt{datafaker} dependency, several changes are observed in the new version.
For instance, the parameters of the \texttt{between} method have been modified; in the previous version, both parameters were of data type \texttt{Date}, while in the new version, \texttt{Timestamp} is used.

This approach allows us to identify all modifications in the new version of the direct dependency that could affect the dependency update process in the client's project.

\todo{what about the cases where there are no changes between the two versions of the direct dep, but the changes are further down in the indirect deps?}


% \begin{itemize}
% \item Number of generated explanations
% \item Number / proportion of correct and incorrect explanations
% \item Number / proportion of missing explanations. Why?
% \item Number / proportion of partial explanations. Why?
% \item Number of errors with and without suggestions
% \end{itemize}    

\tool can be used as a standard command-line tool to generate automatic explanations of the causes of breaking dependency updates.
As input, it takes the code of the client application, the previous version, and the new version of the updated dependency.
On the other hand, it can be directly integrated into the development workflow as a GitHub bot, automating the generation of detailed explanations of build failures due to breaking dependency updates.
\tool as a bot, monitors pull requests where the CI fails and only updates the version for a single dependency.
\tool analyzes build logs to identify errors caused by the update.
Next, compare dependency versions, identifying which elements have been changed in the new version of the dependency.
From the results of the analysis and comparison, \tool identifies the elements of the client application affected by the changes in the new version of the dependency.
Finally, generates the explanation addressing the causes of the dependency update failure,
i) due to the use of elements that belong to direct or indirect dependencies used in the client application code or
ii) due to failures caused by incompatibilities between Java versions or due to specific configurations in the Maven configuration file.

These explanations allow developers to easily access the information needed to address and fix problems caused by dependency updates.

%paragraph 2. problem statement: what problem is Breaking good solving?
%paragraph 3. methodology: how we generate explanations
% paragraph 4. explanations and indirect dependency analysis
% paragraph 5. Results
% list of contributions
% outline


\autoref{tab:compilation-error-counts} presents the 6 error causes triggered by the compilation errors observed in the compilation logs.

\begin{table}[htp]
\caption{List of compilation error causes}
\centering
\rowcolors{2}{gray!10}{white}
\begin{tabular}{lc}
\toprule
Causes  &  \makecell{Number of occurrences } \\ 
\midrule
  cannot find symbol &  204 \\
  \begin{tabular}{@{}l@{}} constructor in class cannot be applied to \\  given types
  \end{tabular} & 114 \\
  package does not exist & 43 \\
  cannot access &  10  \\
  static import only from classes and interfaces & 4 \\
  \begin{tabular}{@{}l@{}}exception is never thrown in body \\ of corresponding try statement
  \end{tabular} & 1 \\
  \bottomrule
 
\end{tabular}
\label{tab:compilation-error-counts}
\end{table}

The \textit{cannot find symbol} error is the most frequent error.
It occurs when the compiler cannot find a variable, method, or class specified in the source code.
The second most common error, \textit{constructor in class cannot be applied to given types}. 
Occurs when an attempt is made to call a constructor with incorrect parameters that do not match any of the constructor signatures defined in the class.
The error \textit{package does not exist} occurs 43 times and is due to references to a package that cannot be found by the compiler.
The error \textit{cannot access} was registered 10 times and is triggered due to visibility or accessibility problems of a class or member.
With 4 occurrences, the error \textit{static import only from classes and interfaces} appears when trying to do a static import from something that is not a class or interface.
Finally, the error \textit{exception is never thrown in body of corresponding try statement} occurred once and occurs when an exception is included in a \texttt{try} block, but the exception is never thrown in the body of the \texttt{try}. 

The results obtained are comparable to those reported by Reyes \cite{reyes2024bump} and Jasura \cite{Jayasuriya2023UnderstandingWild} \todo{do these works also study breakages due to indirect dependencies? or do they look at direct deps and find that the reason for the breakage are similar to the reasons we observe here with indirect deps?}.
The use of indirect dependencies in the client application code induces errors similar to those observed in both studies. \todo{it's strange that an application invokes an indirect dependency. Do previous also observe this? did they look at why applications do this instead of declaring the invoked dep as a direct dep?}
The 6 causes of errors identified in our study are among the 10 most common in both referenced studies.


% \subsection{User study}

% \textbf{Description of the task}

% We ask users to do something about a breaking update, with and without explanations.

% \textbf{Metrics}
% \begin{enumerate}
%     \item Time to resolve the issue
%     \item Number of breakages identified
% \end{enumerate}


% \textbf{Questionnaire}
% \begin{enumerate}
%     \item Likert scale How difficult was it to identify the cause of the breakage?
%     \item Likert scale To what extent do you think the detailed explanation facilitates the identification of the breakage?
%     \item Likert scale How useful did you find the explanation document provided for solving the problem in the compilation process?
%     % \item [Likert scale] How would you rate the usability of the provided explanation document?
%     \item Open question What are the strengths of the approach to your opinion?
%     \item Open question What are the weaknesses of the approach to your opinion?
% \end{enumerate}

% \autoref{fig:indirect_modification} shows the distribution of updated, removed, and added indirect dependencies for each breaking dependency update categorized as \indirectCategory.
% The median number of indirect dependencies added by breaking update is \medianAdded, the median number of indirect dependencies removed is \medianRemoved and the median number of indirect dependencies updated is \medianModified \todo{when you give the median, what is the size of each set? how many of the 41 breakages have at least one indirect dep that is removed/added or updated? how many of these indirect deps added/removed/changed are involved in the breakage? How about having a simpler plot where give the share of the 41 that are due to an indirect dep that is added or removed or modified?}. 
% The distribution shows that indirect dependencies have a significant impact on updating dependencies, adding, deleting, and modifying several of them \todo{I don't understand this sentence. }.
% This indicates that updates are conflicting and cause conflicts in the compilation of the client application code.


%Explanations quantity
Next, we generate explanations for each of the categorized breaking updates.
\autoref{tab:compilation-category-counts} shows the number of explanations generated for each compilation error category.
Each explanation is generated according to the template defined for each compilation error category.
\tool generates a total of 170 explanations for 243 breaking dependency updates that fail due to compilation errors.

\tool generates a total of 82/116 explanations for breaking updates categorized as \directCategory.
The explanations detail the modifications or deletions of constructs in the new version of the dependency and suggest alternatives to resolve the problem.
% The explanations include the identification of the specific methods and classes affected, the lines of code where the errors occur, and possible suggested fixes.
For example, \autoref{fig:explanation} shows the explanation generated for the breaking update of the \texttt{datafaker} dependency from version \texttt{1.3.0} to version \texttt{1.3.0} in project \texttt{flink-flaker}.
The explanation shows how the change in the behavior of the \texttt{between} method causes the breaking update.
The missing explanations are due to japicmp not detecting API changes related to the constructs involved in the compilation errors generated by the breaking update.

In the \javaIncompCategory category, \tool generates 72/72 \todo{72/72 or 2/72 as indicated in the table?. Sorry was a mistake} explanations automatically.
We compared the Java bytecode versions required by the dependency with the JVM used for client compilation.
% The explanations discuss the incompatibility by identifying the Java versions required, indicating the configuration files that need to be updated, and suggesting alternatives to maintain compatibility.
% The explanations include a list of errors extracted from the logs that are caused by Java version incompatibility.
\autoref{fig:java_version_incompatibility_explanation} shows an example of an explanation generated for updating the \texttt{spring-core} dependency from version \texttt{5.3.23} to version \texttt{6.0.3}. The explanation identifies as the cause of the breakage the incompatibility between the versions used in the client compilation (Java 11) and the version required by the dependency (Java 17).

For the \wErrorCategory category, \tool generates 8/8 explanations.
The explanations show the warnings generated by the deprecated constructs in the new version of the dependency.
It also includes the list of files that contain the enabled option.
\autoref{anex_werror} shows the explanation generated for the breaking update of the dependency \texttt{hibernate-entitymanager} from version \texttt{4.2.11.Final} to version \texttt{5.5.14.Final} in the project \texttt{nem}.
The explanation highlights how 4 configuration files contain the enabled option causing the breaking updates.

\tool generates only 2 of 38 possible explanations for broken updates classified as \indirectCategory.
The explanations provide details about the affected indirect dependencies, and the specific constructs causing the errors, and suggest adjustments to the client code to resolve the problems.
\autoref{anex_indirect} shows the dependency update of \texttt{maven-surefire-common} from version \texttt{3.0.0-M5} to version \texttt{3.0.0-M7}.
The upgrade fails due to the update of the indirect dependency \texttt{surefire-api} from version \texttt{3.0.0-M5} to version \texttt{3.0.0-M7}.
The new version of the indirect dependency removes the \texttt{getInstance} method that is used in the client application.
The low number of explanations generated in this category is due to the lack of a clear relationship between the compilation errors and the modified indirect dependencies in the updated dependency.


\appendices
\newpage
\section{\javaIncompCategory explanation example}
\begin{figure}[hpt]
    \centering
    \includegraphics[width=.90\linewidth]{Figure/image 9.pdf}
    \caption{Generated explanation after the breaking dependency update due to \javaIncompCategory.}
    \label{fig:java_version_incompatibility_explanation}
\end{figure}

\newpage
\section{\wErrorCategory explanation example}
\label{anex_werror}
\begin{figure}[hpt]
    \centering
    \includegraphics[width=.80\linewidth]{Figure/image 10 (2).pdf}
    \caption{Generated explanation after the breaking dependency update due to \wErrorCategory.}
    \label{fig:werror_explanation}
\end{figure}

\section{\indirectCategory explanation example}
\label{anex_indirect}
